Loosely Synchronized Search for Multi-agent Path Finding with Asynchronous Actions

Multi-agent path finding (MAPF) determines an ensemble of collision-free paths for multiple agents between their respective start and goal locations. Among the available MAPF planners for workspace modeled as a graph, A*-based approaches have been widely investigated due to their guarantees on completeness and solution optimality, and have demonstrated their efficiency in many scenarios. However, almost all of these A*-based methods assume that each agent executes an action concurrently in that all agents start and stop together. This article presents a natural generalization of MAPF with asynchronous actions (MAPF-AA) where agents do not necessarily start and stop concurrently. The main contribution of the work is a proposed approach called Loosely Synchronized Search (LSS) that extends A*-based MAPF planners to handle asynchronous actions. We show LSS is complete and finds an optimal solution if one exists. We also combine LSS with other existing MAPF methods that aims to trade-off optimality for computational efficiency. Numerical results are presented to corroborate the performance of LSS and the applicability of the proposed method is verified in the Robotarium, a remotely accessible swarm robotics research platform.

==> contents/OUTDATED_main.tex <==
% \def\year{2021}\relax
% %File: formatting-instructions-latex-2021.tex
% %release 2021.2
% \documentclass[letterpaper]{article} % DO NOT CHANGE THIS
% \usepackage{aaai21}  % DO NOT CHANGE THIS
% \usepackage{times}  % DO NOT CHANGE THIS
% \usepackage{helvet} % DO NOT CHANGE THIS
% \usepackage{courier}  % DO NOT CHANGE THIS
% \usepackage[hyphens]{url}  % DO NOT CHANGE THIS
% \usepackage{graphicx} % DO NOT CHANGE THIS
% \urlstyle{rm} % DO NOT CHANGE THIS
% \def\UrlFont{\rm}  % DO NOT CHANGE THIS
% \usepackage{natbib}  % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
% \usepackage{caption} % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
% \frenchspacing  % DO NOT CHANGE THIS
% \setlength{\pdfpagewidth}{8.5in}  % DO NOT CHANGE THIS
% \setlength{\pdfpageheight}{11in}  % DO NOT CHANGE THIS
% %\nocopyright
% %PDF Info Is REQUIRED.
% % For /Author, add all authors within the parentheses, separated by commas. No accents or commands.
% % For /Title, add Title in Mixed Case. No accents or commands. Retain the parentheses.
% \pdfinfo{
% /Title (AAAI Press Formatting Instructions for Authors Using LaTeX -- A Guide)
% /Author (AAAI Press Staff, Pater Patel Schneider, Sunil Issar, J. Scott Penberthy, George Ferguson, Hans Guesgen, Francisco Cruz, Marc Pujol-Gonzalez)
% /TemplateVersion (2021.2)
% } %Leave this
% % /Title ()
% % Put your actual complete title (no codes, scripts, shortcuts, or LaTeX commands) within the parentheses in mixed case
% % Leave the space between \Title and the beginning parenthesis alone
% % /Author ()
% % Put your actual complete list of authors (no codes, scripts, shortcuts, or LaTeX commands) within the parentheses in mixed case.
% % Each author should be only by a comma. If the name contains accents, remove them. If there are any LaTeX commands,
% % remove them.


% %%%%%% My Packages %%%%%%
% \usepackage{graphicx} % for \graphicspath
% \usepackage{subfigure,wrapfig}
% \usepackage{subfigmat}
% \usepackage{algorithm}
% \usepackage[noend]{algpseudocode} % algorithmic, \State{}, etc
% \usepackage{amssymb,amsmath,amsthm}
% %\usepackage{amsthm} % theorem, lemma, etc
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% \newtheorem{definition}{Definition}
% %\newtheorem{proof}{Proof}
% \newtheorem{corollary}{Corollary}
% %%%%%% End of My Packages %%%%%%


% % DISALLOWED PACKAGES
% % \usepackage{authblk} -- This package is specifically forbidden
% % \usepackage{balance} -- This package is specifically forbidden
% % \usepackage{color (if used in text)
% % \usepackage{CJK} -- This package is specifically forbidden
% % \usepackage{float} -- This package is specifically forbidden
% % \usepackage{flushend} -- This package is specifically forbidden
% % \usepackage{fontenc} -- This package is specifically forbidden
% % \usepackage{fullpage} -- This package is specifically forbidden
% % \usepackage{geometry} -- This package is specifically forbidden
% % \usepackage{grffile} -- This package is specifically forbidden
% % \usepackage{hyperref} -- This package is specifically forbidden
% % \usepackage{navigator} -- This package is specifically forbidden
% % (or any other package that embeds links such as navigator or hyperref)
% % \indentfirst} -- This package is specifically forbidden
% % \layout} -- This package is specifically forbidden
% % \multicol} -- This package is specifically forbidden
% % \nameref} -- This package is specifically forbidden
% % \usepackage{savetrees} -- This package is specifically forbidden
% % \usepackage{setspace} -- This package is specifically forbidden
% % \usepackage{stfloats} -- This package is specifically forbidden
% % \usepackage{tabu} -- This package is specifically forbidden
% % \usepackage{titlesec} -- This package is specifically forbidden
% % \usepackage{tocbibind} -- This package is specifically forbidden
% % \usepackage{ulem} -- This package is specifically forbidden
% % \usepackage{wrapfig} -- This package is specifically forbidden
% % DISALLOWED COMMANDS
% % \nocopyright -- Your paper will not be published if you use this command
% % \addtolength -- This command may not be used
% % \balance -- This command may not be used
% % \baselinestretch -- Your paper will not be published if you use this command
% % \clearpage -- No page breaks of any kind may be used for the final version of your paper
% % \columnsep -- This command may not be used
% % \newpage -- No page breaks of any kind may be used for the final version of your paper
% % \pagebreak -- No page breaks of any kind may be used for the final version of your paperr
% % \pagestyle -- This command may not be used
% % \tiny -- This is not an acceptable font size.
% % \vspace{- -- No negative value may be used in proximity of a caption, figure, table, section, subsection, subsubsection, or reference
% % \vskip{- -- No negative value may be used to alter spacing above or below a caption, figure, table, section, subsection, subsubsection, or reference

% \setcounter{secnumdepth}{0} %May be changed to 1 or 2 if section numbers are desired.

% % The file aaai21.sty is the style file for AAAI Press
% % proceedings, working notes, and technical reports.
% %

% % Title

% % Your title must be in mixed case, not sentence case.
% % That means all verbs (including short verbs like be, is, using,and go),
% % nouns, adverbs, adjectives should be capitalized, including both words in hyphenated terms, while
% % articles, conjunctions, and prepositions are lower case unless they
% % directly follow a colon or long dash

% \title{Loosely Synchronized Search for Multi-agent Path Finding with Asynchronous Actions}
% \author {
% 	% Authors
% 	Zhongqiang Ren, \textsuperscript{\rm 1}
% 	Sivakumar Rathinam, \textsuperscript{\rm 2}
% 	Howie Choset \textsuperscript{\rm 1} \\
% }
% \affiliations {
% 	% Affiliations
% 	\textsuperscript{\rm 1} Carnegie Mellon University, 5000 Forbes Ave., Pittsburgh, PA 15213, USA. \\
% 	\textsuperscript{\rm 2} Texas A\&M University, College Station, TX 77843-3123. \\
% 	zhongqir@andrew.cmu.edu, choset@andrew.cmu.edu, srathinam@tamu.edu
% }

% %\title{Loosely Synchronized Search for Multi-agent Path Finding with Different Speeds}
% %\author{Zhongqiang Ren \textsuperscript{\rm 1}, Sivakumar Rathinam \textsuperscript{\rm 2} and Howie Choset \textsuperscript{\rm 1} % <-this % stops a space
% %}
% %\affiliations{
% %    %Afiliations
% %    \textsuperscript{\rm 1} Zhongqiang Ren and Howie Choset are with Carnegie Mellon University, 5000 Forbes Ave., Pittsburgh, PA 15213, USA. \\
% %    \textsuperscript{\rm 1} Sivakumar Rathinam is with Texas A\&M University,
% %    College Station, TX 77843-3123. \\
% %    %If you have multiple authors and multiple affiliations
% %    % use superscripts in text and roman font to identify them.
% %    %For example,
% %
% %    % Sunil Issar, \textsuperscript{\rm 2}
% %    % J. Scott Penberthy, \textsuperscript{\rm 3}
% %    % George Ferguson,\textsuperscript{\rm 4}
% %    % Hans Guesgen, \textsuperscript{\rm 5}.
% %    % Note that the comma should be placed BEFORE the superscript for optimum readability
% %
% %    2275 East Bayshore Road, Suite 160\\
% %    Palo Alto, California 94303\\
% %    % email address must be in roman text type, not monospace or sans serif
% %    publications21@aaai.org
% %
% %    % See more examples next
% %}

% \begin{document}

% \input{temp_explain}

% \maketitle

% \begin{abstract}
% 	\input{abstract}
% \end{abstract}

% \section{Introduction}\label{sec:intro}
% \input{intro}

% \section{Prior Work}\label{sec:prior}
% \input{prior}

% \section{Problem Description}\label{sec:problem}
% \input{problem}

% \section{Loosely Synchronized Search}\label{sec:method}
% \input{method}

% \section{Analysis}\label{sec:analysis}
% \input{analysis}

% \section{Improvements and Extensions}\label{sec:combine_m}
% \input{combi}

% \section{Numerical Results}\label{sec:result}
% \input{result}

% \section{Conclusion}\label{sec:conclude}
% \input{conclude}


% %\bibliographystyle{plain}
% \bibliography{references}


% \end{document}


==> contents/temp_explain.tex <==

\newpage
\section{A Brief Description of State Expansion in Loosely-Synchronized Search}
\subsection{Notations}
\begin{itemize}
	\item Index set $I=\{1,2,\dots,N\}$.
	\item Let $G^i=(V^i,E^i)$ represent the individual graph corresponds to agent $i\in I$.
	\item Let $\mathcal{N}(v), v\in V^i$ represent the adjacent vertices of $v$ in $G^i$.
	\item Let $D^i(v^i_{1}, v^i_2)$ denote the duration for agent $i$ to move through edge $(v^i_{1}, v^i_2) \in E^i$.
	\item Let $(v^i_{start}, v^i_{end})$ denote the start and end vertex for agent $i$, where $v^i_{start}, v^i_{end} \in V^i$.
	\item Let $(t^i_{start}, t^i_{end})$ denote the start and end timestamps for agent $i$ where $t^i_{start}, t^i_{end} \in \mathbb{R}$.
	\item Let $w^i = ( (v^i_{start}, v^i_{end}), (t^i_{start}, t^i_{end}) )$ denote a \emph{spatial-temporal envelop} for agent $i$, which is a tuple of vertex pair, start timestamp and end timestamp.
	\item Let $s = (w^1,w^2, \dots, w^N)$ denote a search state, which is a tuple of $N$ spatial-temporal envelops.
	% \item We use subscripts $k,l$ under a variable to denote a specific one. For example, $s_k$ represents a specific state. 
	%\item Let $W^i_{ngh}(w^i_k)$ denote a set of neighboring spatial temporal envelops of $w^i_k$, where each $w^i_l \in W^i_{ngh}(w^i_k)$ is a neighbor of $w^i$. How to compute $W^i_{ngh}(w^i_k)$ given $w^i_k$ is elaborated later.
\end{itemize}

\subsection{Neighbor Generation}
In Loosely-Synchronized A*, given a state $s$, to compute its neighboring states, the following four steps are conducted in order. %Step (1) and (2) find which agent(s) should take actions based on their ending timestamps in $s$. Step (3) generate individual neighbors for those agenats and Step (4) takes combination of those individual neighbors over all agents to form neighboring states.

\underline{Step (1)} The minimum end timestamp $t^{min}_{end}(s)$ among all agents within $s$ is computed:
\begin{equation}
	t^{min}_{end}(s) = \min_{i\in I} t^i_{end}.
\end{equation}

\underline{Step (2)} The subset of agents $I_{t^{min}_{end}}(s) \subseteq I$ with end timestamp equal to $t_{min}(s)$ is computed:
\begin{equation}
I_{t^{min}_{end}}(s) = \arg\min_{i\in I} t^i_{end}.
\end{equation}

\underline{Step (3)} This step computes individual neighbors for each agent $i \in I$. Let $W^i_{ngh}(w^i)$ represent a set of spatial-temporal envelops generated from $w^i$.
\begin{itemize}
	\item For $i \notin I_{t^{min}_{end}}(s)$, agent $i$ is not allowed to take actions and the spatial-temporal envelop of agent $i$ remains the same as $w^i_k$: $W^i_{ngh}(w^i_k)$ contains $w^i_k$ only.
	
	\item For $i \in I_{t^{min}_{end}}(s)$, agent $i$ is allowed to take actions including wait and move. $W^i_{ngh}(w^i)$ contains $(| \mathcal{N}(v^i_{end})|+1)$ neighbors, where $v^i_{end}$ is the end vertex of agent $i$ in state $s$. 
\end{itemize}
Specifically, to move agent $i$, for each vertex $v'^i \in \mathcal{N}(v^i_{end})$ , a corresponding spatial-temporal envelop $w'^i = ( (v'^i_{start}, v'^i_{end}), (t'^i_{start}, t'^i_{end}) )$ is generated with
\begin{eqnarray}
v'^i_{start} &=& v^i_{end}\\
v'^i_{end }&=& v'^i \\
t'^i_{start} &=& t^i_{end} \\
t'^i_{end} &=& t^i_{end} + D^i(v^i_{end}, v'^i) 
\end{eqnarray}
and $w'^i$ is added to $W^i_{ngh}(w^i_k)$. 

To let agent $i$ wait-in-place, a spatial-temporal envelop $w'^i = ( (v'^i_{start}, v'^i_{end}), (t'^i_{start}, t'^i_{end}) )$ is generated with
\begin{eqnarray}
v'^i_{start} &=& v^i_{end}\\
v'^i_{end }&=& v^i_{end} \\
t'^i_{start} &=& t^i_{end} \\
t'^i_{end} &=& t^i_{end} + D^i_{wait} 
\end{eqnarray}
where $D^i_{wait}$, the amount of wait time, is computed as follows:
\begin{itemize}
	\item If $I_{t^{min}_{end}}(s) = I$ (which means all agents have the same ending timestamps), then let 
	\begin{eqnarray}
	D^i_{wait} =  \min_{i\in I, e\in E^i} D^i(e),
	\end{eqnarray}
	which means agent $i$ waits for a small fraction of time that is the minimum duration of all possible movement of any agents through any edges in the graph.
	\item If $I_{t^{min}_{end}}(s) \neq I$ (which means there is at least one agent in state $s$ whose ending timestamp is larger than $t^{min}_{end}(s)$), then let $I \backslash I_{t^{min}_{end}}(s)$ denote the complement set of $I_{t^{min}_{end}}(s)$ with respect to $I$ and let 
	\begin{eqnarray}
	D^i_{wait} = \min_{i\in I \backslash I_{t^{min}_{end}}(s)} t^i_{end} - t^{min}_{end}(s),
	\end{eqnarray}
	where $\min_{i\in I \backslash I_{t^{min}_{end}}(s)} t^i_{end}$ is basically the second minimum timestamp in state $s$ and the amount of wait time is the different between the second minimum timestamp and the minimum end timestamp in state $s$.
\end{itemize}

\underline{Step (4)} Take combination of $W^i_{ngh}$ over all agents $i \in I$ and the set of neighboring state of $s$ is generated.

\subsection{Remark}
Given a state $s$, if $I_{t^{min}_{end}}(s) = I$ (which means all agents have the same ending timestamps), state $s$ is defined to be a \emph{synchronized} state.
\begin{definition}
	A state $s$ is a synchronized state, if $t(s^i)=t(s^j), \forall i,j \in I, i\neq j$.
\end{definition}
%Given a state $s$, let $v_{end}(s)$ denote a joint vertex that is formed by each agent's end vertex: $v_{end}(s) = (v^1_{end}, v^2_{end}, \dots v^N_{end})$. 
%The neighbor generation procedure described above guarantees the generation of a synchronized state at joint vertex $v_{end}(s) = v$
